Controlling Learned Effects to Reduce Spurious Correlations in Text Classifiers

To address the problem of NLP classifiers learning spurious correlations between training features and target labels, a common approach is to make the model's predictions invariant to these features. However, this can be counter-productive when the features have a non-zero causal effect on the target label and thus are important for prediction. Therefore, using methods from the causal inference literature, we propose an algorithm to regularize the learnt effect of the features on the model's prediction to the estimated effect of feature on label. This results in an automated augmentation method that leverages the estimated effect of a feature to appropriately change the labels for new augmented inputs. On toxicity and IMDB review datasets, the proposed algorithm minimises spurious correlations and improves the minority group (i.e., samples breaking spurious correlations) accuracy, while also improving the total accuracy compared to standard training.

==> files/cutout.tex <==

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}
\section{Preamble}
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{ct1965} & \verb|\citep| & \verb|\cite| \\
\citealp{ct1965} & \verb|\citealp| & no equivalent \\
\citet{ct1965} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{ct1965} & \verb|\citeyearpar| & \verb|\shortcite| \\
\citeposs{ct1965} & \verb|\citeposs| & no equivalent \\
\citep[FFT;][]{ct1965} &  \verb|\citep[FFT;][]| & no equivalent\\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}
The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}
To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{ACL2023}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{ACL2023}
\end{verbatim}
\end{quote}
To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)
Please see the \LaTeX{} source of this document for comments on other packages that may be useful.
Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.
By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,augenstein-etal-2016-stance,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}
You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}
Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.


==> tables/cer_accuracies_combined_bert.tex <==
\begin{table*}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l||llll|HHllH|}
\hline
Method & Group1 & Group2 & Group3 & Group4 & Treatment0 & Treatment1 & Total & Avg Group & Direct \\
\hline
\stdfine & 99.46 $\pm$ 0.08  & 3.52 $\pm$ 0.80  & 1.61 $\pm$ 0.29  & 99.42 $\pm$ 0.10  & 88.30 $\pm$ 0.03  & 87.25 $\pm$ 0.02  & 87.77 $\pm$ 0.02  & 51.00 $\pm$ 0.17  & 59.43 $\pm$ 1.28  \\
\removetoken & 88.71 $\pm$ 0.75  & 28.06 $\pm$ 0.94  & 37.46 $\pm$ 2.36  & 90.69 $\pm$ 0.85  & 82.86 $\pm$ 0.46  & 82.74 $\pm$ 0.62  & 82.80 $\pm$ 0.14  & 61.23 $\pm$ 0.45  & 1.43 $\pm$ 0.13  \\
\hline
\dfl & 72.45 $\pm$ 1.33  & 35.62 $\pm$ 5.51  & 53.58 $\pm$ 2.61  & 82.46 $\pm$ 3.38  & 70.30 $\pm$ 0.95  & 76.51 $\pm$ 2.25  & 73.45 $\pm$ 0.76  & 61.03 $\pm$ 0.77  & 3.78 $\pm$ 1.53  \\
\dflsuccess & 99.22 $\pm$ 0.34  & 4.13 $\pm$ 1.21  & 3.12 $\pm$ 0.92  & 99.34 $\pm$ 0.18  & 88.26 $\pm$ 0.21  & 87.25 $\pm$ 0.01  & 87.75 $\pm$ 0.10  & 51.45 $\pm$ 0.41  & 56.99 $\pm$ 2.67  \\
\poe & 100.00 $\pm$ 0.00  & 0.18 $\pm$ 0.14  & 0.00 $\pm$ 0.00  & 99.96 $\pm$ 0.02  & 88.59 $\pm$ 0.00  & 87.30 $\pm$ 0.02  & 87.94 $\pm$ 0.01  & 50.03 $\pm$ 0.03  & 74.95 $\pm$ 2.60  \\
\hline
\inlp & 79.10 $\pm$ 3.75  & 73.44 $\pm$ 7.52  & 38.77 $\pm$ 7.53  & 36.35 $\pm$ 9.45  & 74.50 $\pm$ 2.50  & 41.06 $\pm$ 7.31  & 57.54 $\pm$ 2.48  & 56.92 $\pm$ 1.41  & 59.62 $\pm$ 3.91  \\
\hline
\subsample & 85.45 $\pm$ 3.98  & 59.89 $\pm$ 8.49  & 27.59 $\pm$ 8.76  & 57.72 $\pm$ 9.77  & 78.85 $\pm$ 2.53  & 57.99 $\pm$ 7.46  & 68.27 $\pm$ 2.54  & 57.66 $\pm$ 1.55  & 3.25 $\pm$ 1.35  \\
\groupdro & 63.98 $\pm$ 4.43  & 43.18 $\pm$ 4.68  & 59.42 $\pm$ 4.75  & 72.19 $\pm$ 3.31  & 63.46 $\pm$ 3.38  & 68.51 $\pm$ 2.30  & 66.02 $\pm$ 0.97  & 59.69 $\pm$ 0.28  & 7.91 $\pm$ 0.81  \\
\hline
\cer{0} & 98.89 $\pm$ 0.48  & 7.48 $\pm$ 1.77  & 4.03 $\pm$ 1.53  & 97.40 $\pm$ 0.76  & 88.07 $\pm$ 0.29  & 85.99 $\pm$ 0.44  & 87.01 $\pm$ 0.34  & 51.95 $\pm$ 0.31  & 47.04 $\pm$ 3.88  \\
\cer{ate} & 98.30 $\pm$ 0.30  & 4.13 $\pm$ 0.94  & 7.75 $\pm$ 1.28  & 99.36 $\pm$ 0.18  & 87.97 $\pm$ 0.14  & 87.27 $\pm$ 0.06  & 87.62 $\pm$ 0.06  & 52.39 $\pm$ 0.16  & 51.59 $\pm$ 0.18  \\
\hline
\hline
\stdfine & 76.72 $\pm$ 0.82  & 5.80 $\pm$ 1.57  & 81.72 $\pm$ 0.91  & 96.72 $\pm$ 0.35  & 79.16 $\pm$ 0.36  & 79.92 $\pm$ 0.19  & 79.38 $\pm$ 0.29  & 65.24 $\pm$ 0.31  & 18.46 $\pm$ 0.35  \\
\removetoken & 75.63 $\pm$ 0.79  & 15.22 $\pm$ 1.02  & 83.10 $\pm$ 0.43  & 90.15 $\pm$ 0.61  & 79.27 $\pm$ 0.33  & 76.31 $\pm$ 0.33  & 78.40 $\pm$ 0.23  & 66.02 $\pm$ 0.28  & 10.20 $\pm$ 0.09  \\
\hline
\dfl & 83.28 $\pm$ 0.16  & 9.42 $\pm$ 0.59  & 67.82 $\pm$ 0.66  & 94.09 $\pm$ 0.80  & 75.74 $\pm$ 0.33  & 78.45 $\pm$ 0.61  & 76.54 $\pm$ 0.36  & 63.65 $\pm$ 0.24  & 17.53 $\pm$ 0.78  \\
\dflsuccess & 78.80 $\pm$ 1.84  & 3.62 $\pm$ 1.18  & 77.82 $\pm$ 2.34  & 97.54 $\pm$ 0.46  & 78.32 $\pm$ 0.21  & 80.19 $\pm$ 0.22  & 78.87 $\pm$ 0.21  & 64.44 $\pm$ 0.20  & 19.52 $\pm$ 0.52  \\
\poe & 79.02 $\pm$ 0.62  & 10.14 $\pm$ 1.57  & 79.43 $\pm$ 0.66  & 95.24 $\pm$ 0.71  & 79.22 $\pm$ 0.57  & 79.52 $\pm$ 0.33  & 79.30 $\pm$ 0.37  & 65.96 $\pm$ 0.52  & 17.57 $\pm$ 1.06  \\
\hline
\inlp & 69.02 $\pm$ 1.04  & 6.52 $\pm$ 2.51  & 88.45 $\pm$ 0.10  & 95.07 $\pm$ 0.57  & 78.49 $\pm$ 0.49  & 78.71 $\pm$ 0.00  & 78.55 $\pm$ 0.34  & 64.77 $\pm$ 0.25  & 18.88 $\pm$ 0.10  \\
\hline
\subsample & 73.99 $\pm$ 0.32  & 28.26 $\pm$ 2.72  & 83.45 $\pm$ 1.14  & 84.40 $\pm$ 0.97  & 78.60 $\pm$ 0.51  & 74.03 $\pm$ 0.29  & 77.25 $\pm$ 0.45  & 67.52 $\pm$ 0.17  & 1.80 $\pm$ 0.14  \\
\groupdro & 78.14 $\pm$ 1.32  & 44.93 $\pm$ 4.27  & 73.45 $\pm$ 5.25  & 71.92 $\pm$ 2.36  & 75.85 $\pm$ 2.03  & 66.93 $\pm$ 1.26  & 73.22 $\pm$ 1.79  & 67.11 $\pm$ 1.20  & 0.11 $\pm$ 1.65  \\
\hline
\cer{0} & 78.25 $\pm$ 0.45  & 11.59 $\pm$ 1.18  & 79.43 $\pm$ 0.25  & 94.25 $\pm$ 0.35  & 78.82 $\pm$ 0.16  & 78.98 $\pm$ 0.39  & 78.87 $\pm$ 0.14  & 65.88 $\pm$ 0.28  & 9.25 $\pm$ 0.42  \\
\cer{ate} & 78.80 $\pm$ 0.32  & 10.14 $\pm$ 0.59  & 80.34 $\pm$ 0.32  & 95.73 $\pm$ 0.35  & 79.55 $\pm$ 0.30  & 79.92 $\pm$ 0.19  & 79.66 $\pm$ 0.17  & 66.25 $\pm$ 0.22  & 14.92 $\pm$ 0.19  \\
\hline
\hline
\stdfine & 98.53 $\pm$ 0.73  & 5.82 $\pm$ 2.16  & 20.78 $\pm$ 8.84  & 99.87 $\pm$ 0.05  & 88.52 $\pm$ 0.57  & 89.47 $\pm$ 0.22  & 88.98 $\pm$ 0.38  & 56.25 $\pm$ 2.25  & 71.93 $\pm$ 5.41  \\
\removetoken & 81.96 $\pm$ 1.69  & 79.37 $\pm$ 1.98  & 69.26 $\pm$ 1.77  & 76.73 $\pm$ 2.67  & 80.32 $\pm$ 1.30  & 77.02 $\pm$ 2.17  & 78.71 $\pm$ 0.82  & 76.83 $\pm$ 0.50  & 0.46 $\pm$ 0.09  \\
\hline
\dfl & 96.87 $\pm$ 1.27  & 8.99 $\pm$ 6.72  & 30.30 $\pm$ 9.52  & 99.28 $\pm$ 0.51  & 88.29 $\pm$ 0.28  & 89.30 $\pm$ 0.30  & 88.78 $\pm$ 0.29  & 58.86 $\pm$ 3.00  & 70.05 $\pm$ 3.84  \\
\dflsuccess & 94.82 $\pm$ 0.94  & 7.41 $\pm$ 3.54  & 41.56 $\pm$ 5.34  & 99.67 $\pm$ 0.27  & 87.96 $\pm$ 0.16  & 89.47 $\pm$ 0.17  & 88.70 $\pm$ 0.00  & 60.86 $\pm$ 1.71  & 63.59 $\pm$ 4.03  \\
\poe & 98.59 $\pm$ 0.84  & 14.29 $\pm$ 8.51  & 24.68 $\pm$ 4.25  & 98.82 $\pm$ 0.97  & 89.07 $\pm$ 0.18  & 89.47 $\pm$ 0.14  & 89.27 $\pm$ 0.16  & 59.09 $\pm$ 1.51  & 69.40 $\pm$ 3.60  \\
\hline
\inlp & 68.33 $\pm$ 4.57  & 58.73 $\pm$ 14.62  & 49.78 $\pm$ 6.50  & 50.43 $\pm$ 14.88  & 65.94 $\pm$ 3.87  & 51.35 $\pm$ 11.72  & 58.82 $\pm$ 5.45  & 56.82 $\pm$ 1.34  & 68.26 $\pm$ 3.99  \\
\hline
\subsample & 71.53 $\pm$ 3.64  & 65.08 $\pm$ 1.98  & 74.46 $\pm$ 2.90  & 85.67 $\pm$ 2.94  & 71.91 $\pm$ 2.80  & 83.39 $\pm$ 2.40  & 77.51 $\pm$ 0.28  & 74.18 $\pm$ 0.09  & 2.86 $\pm$ 0.21  \\
\groupdro & 79.40 $\pm$ 3.67  & 55.56 $\pm$ 2.70  & 67.97 $\pm$ 1.97  & 90.66 $\pm$ 0.82  & 77.93 $\pm$ 2.95  & 86.78 $\pm$ 0.50  & 82.25 $\pm$ 1.34  & 73.40 $\pm$ 0.51  & 17.07 $\pm$ 2.56  \\
\hline
\cer{0} & 94.63 $\pm$ 0.72  & 33.33 $\pm$ 7.23  & 46.75 $\pm$ 1.84  & 97.30 $\pm$ 1.09  & 88.46 $\pm$ 0.47  & 90.23 $\pm$ 0.24  & 89.33 $\pm$ 0.15  & 68.00 $\pm$ 1.65  & 44.84 $\pm$ 2.76  \\
\cer{ate} & 95.46 $\pm$ 1.27  & 15.34 $\pm$ 3.03  & 43.29 $\pm$ 5.49  & 99.34 $\pm$ 0.28  & 88.74 $\pm$ 0.43  & 90.06 $\pm$ 0.13  & 89.38 $\pm$ 0.16  & 63.36 $\pm$ 1.75  & 57.26 $\pm$ 2.88  \\
\hline
\end{tabular}
}
\caption{\label{tab:ceracc_combined_bert}
IMDB BERT
}
\end{table*}


